Mapping Election Polarization and Competitiveness using Election Results

The simplified hypothesis that an election is polarized as an explanation of recent electoral outcomes worldwide is centered on perceptions of voting patterns rather than ideological data from the electorate. While the literature focuses on measuring polarization using ideological-like data from electoral studies-which are limited to economically advantageous countries and are representative mostly to national scales-we argue that, in fact, voting patterns can lead to mapping effective proxies of citizen divisions on election day. This paper perspectives two complementary concepts, Election Polarization (EP) and Election Competitiveness (EC), as a means to understand voting patterns on Election Day. We present an agnostic approach that relies solely on election data and validate it using synthetic and real-world election data across 13 countries in the Eurozone, North America, Latin America, and New Zealand. Overall, we find that we can label and distinguish expectations of polarized and competitive elections in these countries, and we report that EP positively correlates with a metric of political polarization in the U.S., unlocking opportunities for studies of polarization at the regional level and for lower/middle-income countries where electoral studies are available, but surveys are limited.

==> Supplementary_Tables/Between-EPI-current.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
Between-EP (t - 1)            & $0.74^{***}$ &          &          &            &          &             &             & $0.71^{***}$ & $0.72^{***}$ \\
                              & $(0.07)$     &          &          &            &          &             &             & $(0.08)$     & $(0.08)$     \\
Inequality level (t)          &              & $-0.23$  &          &            &          &             & $-0.30$     & $-0.01$      & $-0.01$      \\
                              &              & $(0.29)$ &          &            &          &             & $(0.29)$    & $(0.12)$     & $(0.12)$     \\
Unemployment (t)              &              &          & $0.07$   &            &          &             &             & $0.18$       & $0.18$       \\
                              &              &          & $(0.61)$ &            &          &             &             & $(0.23)$     & $(0.23)$     \\
Spatial Between-EP (t)        &              &          &          & $0.08^{*}$ &          &             &             & $0.02$       & $0.02$       \\
                              &              &          &          & $(0.05)$   &          &             &             & $(0.02)$     & $(0.03)$     \\
Ed. Attainment (t)            &              &          &          &            & $0.15$   &             &             &              & $0.02$       \\
                              &              &          &          &            & $(0.26)$ &             &             &              & $(0.12)$     \\
Log of personal Income PC (t) &              &          &          &            &          & $0.26^{*}$  & $0.27^{**}$ & $0.09$       & $0.09$       \\
                              &              &          &          &            &          & $(0.14)$    & $(0.14)$    & $(0.06)$     & $(0.07)$     \\
Log of GDP PC (t)             & $0.01$       & $-0.01$  & $-0.01$  & $0.01$     & $-0.03$  & $-0.18^{*}$ & $-0.19^{*}$ & $-0.04$      & $-0.04$      \\
                              & $(0.02)$     & $(0.04)$ & $(0.05)$ & $(0.05)$   & $(0.07)$ & $(0.10)$    & $(0.10)$    & $(0.04)$     & $(0.04)$     \\
Log of Pop. Density (t)       & $-0.00$      & $0.01$   & $0.01$   & $0.01$     & $0.01$   & $0.00$      & $0.00$      & $-0.00$      & $-0.00$      \\
                              & $(0.00)$     & $(0.01)$ & $(0.01)$ & $(0.01)$   & $(0.01)$ & $(0.01)$    & $(0.01)$    & $(0.00)$     & $(0.00)$     \\
\hline
Num. obs.                     & $250$        & $300$    & $300$    & $300$      & $300$    & $300$       & $300$       & $250$        & $250$        \\
R$^2$ (full model)            & $0.62$       & $0.15$   & $0.15$   & $0.17$     & $0.15$   & $0.19$      & $0.20$      & $0.62$       & $0.62$       \\
R$^2$ (proj model)            & $0.57$       & $0.03$   & $0.02$   & $0.05$     & $0.03$   & $0.07$      & $0.09$      & $0.58$       & $0.58$       \\
Adj. R$^2$ (full model)       & $0.61$       & $0.13$   & $0.12$   & $0.15$     & $0.13$   & $0.17$      & $0.18$      & $0.61$       & $0.60$       \\
Adj. R$^2$ (proj model)       & $0.56$       & $0.00$   & $-0.01$  & $0.02$     & $-0.00$  & $0.04$      & $0.06$      & $0.56$       & $0.56$       \\
Num. groups: year             & $5$          & $6$      & $6$      & $6$        & $6$      & $6$         & $6$         & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Between-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:between_epi_2}
\end{center}
\end{table}



==> Supplementary_Tables/Between-EPI-v2.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 \\
\hline
Inequality level (t - 1)          & $-0.17$  &          &          &          &          & $-0.19$  & $-0.32$     & $-0.31$     \\
                                  & $(0.31)$ &          &          &          &          & $(0.30)$ & $(0.29)$    & $(0.27)$    \\
Unemployment (t - 1)              &          & $0.57$   &          &          &          &          & $1.30^{**}$ & $1.31^{**}$ \\
                                  &          & $(0.65)$ &          &          &          &          & $(0.58)$    & $(0.57)$    \\
Spatial Between-EP (t - 1)        &          &          & $0.06$   &          &          &          & $0.10^{**}$ & $0.10^{**}$ \\
                                  &          &          & $(0.05)$ &          &          &          & $(0.04)$    & $(0.04)$    \\
Ed. Attainment (t - 1)            &          &          &          & $0.16$   &          &          &             & $0.06$      \\
                                  &          &          &          & $(0.18)$ &          &          &             & $(0.32)$    \\
Log of personal Income PC (t - 1) &          &          &          &          & $0.05$   & $0.05$   & $0.12$      & $0.11$      \\
                                  &          &          &          &          & $(0.07)$ & $(0.07)$ & $(0.08)$    & $(0.14)$    \\
Log of GDP PC (t - 1)             & $0.00$   & $-0.00$  & $0.00$   & $0.00$   & $0.00$   & $0.00$   & $-0.00$     & $-0.00$     \\
                                  & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$    & $(0.01)$    \\
Log of Pop. Density (t - 1)       & $0.00$   & $0.01$   & $0.00$   & $0.00$   & $0.00$   & $0.00$   & $-0.00$     & $-0.00$     \\
                                  & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$    & $(0.01)$    \\
\hline
Num. obs.                         & $250$    & $250$    & $250$    & $250$    & $250$    & $250$    & $250$       & $250$       \\
R$^2$ (full model)                & $0.12$   & $0.13$   & $0.13$   & $0.13$   & $0.13$   & $0.13$   & $0.19$      & $0.19$      \\
R$^2$ (proj model)                & $0.02$   & $0.02$   & $0.03$   & $0.02$   & $0.02$   & $0.03$   & $0.09$      & $0.09$      \\
Adj. R$^2$ (full model)           & $0.10$   & $0.10$   & $0.11$   & $0.10$   & $0.10$   & $0.10$   & $0.15$      & $0.15$      \\
Adj. R$^2$ (proj model)           & $-0.01$  & $-0.01$  & $0.00$   & $-0.01$  & $-0.01$  & $-0.00$  & $0.05$      & $0.05$      \\
Num. groups: year                 & $5$      & $5$      & $5$      & $5$      & $5$      & $5$      & $5$         & $5$         \\
\hline
\multicolumn{9}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Between-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:between_epi_3}
\end{center}
\end{table}



==> Supplementary_Tables/Between-EPI.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
Between-EP (t - 1)                & $0.74^{***}$ &          &          &          &          &          &          & $0.74^{***}$ & $0.74^{***}$ \\
                                  & $(0.07)$     &          &          &          &          &          &          & $(0.08)$     & $(0.08)$     \\
Inequality level (t - 1)          &              & $-0.17$  &          &          &          &          & $-0.19$  & $0.02$       & $0.05$       \\
                                  &              & $(0.31)$ &          &          &          &          & $(0.30)$ & $(0.09)$     & $(0.10)$     \\
Unemployment (t - 1)              &              &          & $0.57$   &          &          &          &          & $1.02^{***}$ & $1.04^{***}$ \\
                                  &              &          & $(0.65)$ &          &          &          &          & $(0.31)$     & $(0.33)$     \\
Spatial Between-EP (t - 1)        &              &          &          & $0.06$   &          &          &          & $0.01$       & $0.01$       \\
                                  &              &          &          & $(0.05)$ &          &          &          & $(0.02)$     & $(0.02)$     \\
Ed. Attainment (t - 1)            &              &          &          &          & $0.16$   &          &          &              & $0.21$       \\
                                  &              &          &          &          & $(0.18)$ &          &          &              & $(0.13)$     \\
Log of personal Income PC (t - 1) &              &          &          &          &          & $0.05$   & $0.05$   & $0.05$       & $0.00$       \\
                                  &              &          &          &          &          & $(0.07)$ & $(0.07)$ & $(0.03)$     & $(0.05)$     \\
Log of GDP PC (t - 1)             & $0.00$       & $0.00$   & $-0.00$  & $0.00$   & $0.00$   & $0.00$   & $0.00$   & $-0.00$      & $-0.00$      \\
                                  & $(0.00)$     & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.00)$     & $(0.00)$     \\
Log of Pop. Density (t - 1)       & $-0.00$      & $0.00$   & $0.01$   & $0.00$   & $0.00$   & $0.00$   & $0.00$   & $-0.00$      & $-0.00$      \\
                                  & $(0.00)$     & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.00)$     & $(0.00)$     \\
\hline
Num. obs.                         & $250$        & $250$    & $250$    & $250$    & $250$    & $250$    & $250$    & $250$        & $250$        \\
R$^2$ (full model)                & $0.62$       & $0.12$   & $0.13$   & $0.13$   & $0.13$   & $0.13$   & $0.13$   & $0.64$       & $0.64$       \\
R$^2$ (proj model)                & $0.57$       & $0.02$   & $0.02$   & $0.03$   & $0.02$   & $0.02$   & $0.03$   & $0.59$       & $0.60$       \\
Adj. R$^2$ (full model)           & $0.60$       & $0.10$   & $0.10$   & $0.11$   & $0.10$   & $0.10$   & $0.10$   & $0.62$       & $0.62$       \\
Adj. R$^2$ (proj model)           & $0.56$       & $-0.01$  & $-0.01$  & $0.00$   & $-0.01$  & $-0.01$  & $-0.00$  & $0.57$       & $0.58$       \\
Num. groups: year                 & $5$          & $5$      & $5$      & $5$      & $5$      & $5$      & $5$      & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Between-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:between_epi_1}
\end{center}
\end{table}



==> Supplementary_Tables/EPI-current.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
EP (t - 1)                    & $0.72^{***}$ &          &          &          &          &          &          & $0.70^{***}$ & $0.69^{***}$ \\
                              & $(0.05)$     &          &          &          &          &          &          & $(0.07)$     & $(0.06)$     \\
Inequality level (t)          &              & $-0.07$  &          &          &          &          & $-0.05$  & $0.00$       & $0.02$       \\
                              &              & $(0.28)$ &          &          &          &          & $(0.28)$ & $(0.12)$     & $(0.12)$     \\
Unemployment (t)              &              &          & $0.36$   &          &          &          &          & $0.03$       & $0.05$       \\
                              &              &          & $(0.43)$ &          &          &          &          & $(0.29)$     & $(0.28)$     \\
Spatial EP (t)                &              &          &          & $0.12$   &          &          &          & $0.04$       & $0.04$       \\
                              &              &          &          & $(0.07)$ &          &          &          & $(0.04)$     & $(0.04)$     \\
Ed. Attainment (t)            &              &          &          &          & $-0.05$  &          &          &              & $0.12$       \\
                              &              &          &          &          & $(0.25)$ &          &          &              & $(0.12)$     \\
Log of personal Income PC (t) &              &          &          &          &          & $-0.09$  & $-0.09$  & $-0.05$      & $-0.09^{*}$  \\
                              &              &          &          &          &          & $(0.10)$ & $(0.10)$ & $(0.05)$     & $(0.05)$     \\
Log of GDP PC (t)             & $0.01$       & $-0.02$  & $-0.01$  & $0.02$   & $-0.01$  & $0.04$   & $0.04$   & $0.05$       & $0.06$       \\
                              & $(0.02)$     & $(0.04)$ & $(0.05)$ & $(0.06)$ & $(0.07)$ & $(0.08)$ & $(0.08)$ & $(0.04)$     & $(0.04)$     \\
Log of Pop. Density (t)       & $-0.00$      & $0.01$   & $0.01$   & $0.01$   & $0.01$   & $0.01$   & $0.01$   & $-0.00$      & $-0.00$      \\
                              & $(0.00)$     & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.01)$ & $(0.00)$     & $(0.00)$     \\
\hline
Num. obs.                     & $250$        & $300$    & $300$    & $300$    & $300$    & $300$    & $300$    & $250$        & $250$        \\
R$^2$ (full model)            & $0.55$       & $0.03$   & $0.03$   & $0.10$   & $0.03$   & $0.03$   & $0.03$   & $0.55$       & $0.56$       \\
R$^2$ (proj model)            & $0.55$       & $0.03$   & $0.03$   & $0.10$   & $0.03$   & $0.03$   & $0.03$   & $0.55$       & $0.56$       \\
Adj. R$^2$ (full model)       & $0.53$       & $0.00$   & $0.00$   & $0.08$   & $-0.00$  & $0.01$   & $0.00$   & $0.53$       & $0.53$       \\
Adj. R$^2$ (proj model)       & $0.53$       & $-0.00$  & $0.00$   & $0.07$   & $-0.00$  & $0.01$   & $0.00$   & $0.53$       & $0.53$       \\
Num. groups: year             & $5$          & $6$      & $6$      & $6$      & $6$      & $6$      & $6$      & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:epi_2}
\end{center}
\end{table}



==> Supplementary_Tables/EPI-v2.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 \\
\hline
Inequality level (t - 1)          & $-0.38^{*}$  &              &              &              &              & $-0.36^{*}$  & $-0.49^{**}$ & $-0.46^{**}$ \\
                                  & $(0.22)$     &              &              &              &              & $(0.21)$     & $(0.21)$     & $(0.21)$     \\
Unemployment (t - 1)              &              & $0.71$       &              &              &              &              & $1.08$       & $1.12^{*}$   \\
                                  &              & $(0.56)$     &              &              &              &              & $(0.66)$     & $(0.66)$     \\
Spatial EP (t - 1)                &              &              & $0.07$       &              &              &              & $0.09$       & $0.09$       \\
                                  &              &              & $(0.07)$     &              &              &              & $(0.06)$     & $(0.06)$     \\
Spatial EP (t - 1)                &              &              & $0.07$       &              &              &              & $0.09$       & $0.09$       \\
                                  &              &              & $(0.07)$     &              &              &              & $(0.06)$     & $(0.06)$     \\
Ed. Attainment (t - 1)            &              &              &              & $0.01$       &              &              &              & $0.24$       \\
                                  &              &              &              & $(0.15)$     &              &              &              & $(0.25)$     \\
Log of personal Income PC (t - 1) &              &              &              &              & $-0.05$      & $-0.04$      & $0.03$       & $-0.02$      \\
                                  &              &              &              &              & $(0.06)$     & $(0.05)$     & $(0.07)$     & $(0.10)$     \\
Log of GDP PC (t - 1)             & $0.05^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.05^{***}$ & $0.04^{***}$ & $0.04^{***}$ \\
                                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     \\
Log of Pop. Density (t - 1)       & $-0.02^{**}$ & $-0.01$      & $-0.01^{*}$  & $-0.01$      & $-0.01$      & $-0.01^{*}$  & $-0.02^{**}$ & $-0.02^{**}$ \\
                                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     \\
\hline
Num. obs.                         & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        \\
R$^2$ (full model)                & $0.26$       & $0.25$       & $0.27$       & $0.24$       & $0.25$       & $0.27$       & $0.32$       & $0.33$       \\
R$^2$ (proj model)                & $0.26$       & $0.25$       & $0.27$       & $0.24$       & $0.25$       & $0.27$       & $0.32$       & $0.33$       \\
Adj. R$^2$ (full model)           & $0.24$       & $0.23$       & $0.25$       & $0.22$       & $0.22$       & $0.24$       & $0.29$       & $0.30$       \\
Adj. R$^2$ (proj model)           & $0.24$       & $0.23$       & $0.25$       & $0.21$       & $0.22$       & $0.24$       & $0.29$       & $0.29$       \\
Num. groups: year                 & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          \\
\hline
\multicolumn{9}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:epi_3}
\end{center}
\end{table}



==> Supplementary_Tables/EPI.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
EP (t - 1)                        & $0.64^{***}$ &              &              &              &              &              &              & $0.61^{***}$ & $0.61^{***}$ \\
                                  & $(0.06)$     &              &              &              &              &              &              & $(0.08)$     & $(0.07)$     \\
Inequality level (t - 1)          &              & $-0.38^{*}$  &              &              &              &              & $-0.36^{*}$  & $-0.14$      & $-0.11$      \\
                                  &              & $(0.22)$     &              &              &              &              & $(0.21)$     & $(0.10)$     & $(0.10)$     \\
Unemployment (t - 1)              &              &              & $0.71$       &              &              &              &              & $0.84^{*}$   & $0.89^{**}$  \\
                                  &              &              & $(0.56)$     &              &              &              &              & $(0.43)$     & $(0.44)$     \\
Spatial EP (t - 1)                &              &              &              & $0.07$       &              &              &              & $0.03$       & $0.03$       \\
                                  &              &              &              & $(0.07)$     &              &              &              & $(0.04)$     & $(0.04)$     \\
Spatial EP (t - 1)                &              &              &              & $0.07$       &              &              &              & $0.03$       & $0.03$       \\
                                  &              &              &              & $(0.07)$     &              &              &              & $(0.04)$     & $(0.04)$     \\
Ed. Attainment (t - 1)            &              &              &              &              & $0.01$       &              &              &              & $0.25^{*}$   \\
                                  &              &              &              &              & $(0.15)$     &              &              &              & $(0.13)$     \\
Log of personal Income PC (t - 1) &              &              &              &              &              & $-0.05$      & $-0.04$      & $0.02$       & $-0.04$      \\
                                  &              &              &              &              &              & $(0.06)$     & $(0.05)$     & $(0.04)$     & $(0.04)$     \\
Log of GDP PC (t - 1)             & $0.02^{**}$  & $0.05^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.05^{***}$ & $0.01^{**}$  & $0.01^{**}$  \\
                                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     \\
Log of Pop. Density (t - 1)       & $-0.01^{**}$ & $-0.02^{**}$ & $-0.01$      & $-0.01^{*}$  & $-0.01$      & $-0.01$      & $-0.01^{*}$  & $-0.01^{**}$ & $-0.01^{**}$ \\
                                  & $(0.00)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.00)$     \\
\hline
Num. obs.                         & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        \\
R$^2$ (full model)                & $0.57$       & $0.26$       & $0.25$       & $0.27$       & $0.24$       & $0.25$       & $0.27$       & $0.59$       & $0.60$       \\
R$^2$ (proj model)                & $0.57$       & $0.26$       & $0.25$       & $0.27$       & $0.24$       & $0.25$       & $0.27$       & $0.59$       & $0.60$       \\
Adj. R$^2$ (full model)           & $0.56$       & $0.24$       & $0.23$       & $0.25$       & $0.22$       & $0.22$       & $0.24$       & $0.57$       & $0.58$       \\
Adj. R$^2$ (proj model)           & $0.56$       & $0.24$       & $0.23$       & $0.25$       & $0.21$       & $0.22$       & $0.24$       & $0.57$       & $0.57$       \\
Num. groups: year                 & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:epi_1}
\end{center}
\end{table}



==> Supplementary_Tables/Within-EPI-current.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
Within-EP (t - 1)             & $1.02^{***}$ &          &          &              &          &               &               & $1.00^{***}$ & $0.99^{***}$ \\
                              & $(0.02)$     &          &          &              &          &               &               & $(0.02)$     & $(0.02)$     \\
Inequality level (t)          &              & $0.16$   &          &              &          &               & $0.25$        & $-0.06$      & $-0.06$      \\
                              &              & $(0.24)$ &          &              &          &               & $(0.23)$      & $(0.04)$     & $(0.04)$     \\
Unemployment (t)              &              &          & $0.29$   &              &          &               &               & $-0.12$      & $-0.11$      \\
                              &              &          & $(0.52)$ &              &          &               &               & $(0.10)$     & $(0.10)$     \\
Spatial Within-EP (t)         &              &          &          & $0.52^{***}$ &          &               &               & $0.06^{**}$  & $0.07^{**}$  \\
                              &              &          &          & $(0.13)$     &          &               &               & $(0.03)$     & $(0.03)$     \\
Ed. Attainment (t)            &              &          &          &              & $-0.20$  &               &               &              & $0.02$       \\
                              &              &          &          &              & $(0.22)$ &               &               &              & $(0.04)$     \\
Log of personal Income PC (t) &              &          &          &              &          & $-0.35^{***}$ & $-0.37^{***}$ & $-0.02$      & $-0.03$      \\
                              &              &          &          &              &          & $(0.12)$      & $(0.12)$      & $(0.02)$     & $(0.02)$     \\
Log of GDP PC (t)             & $-0.00$      & $-0.01$  & $-0.00$  & $0.06$       & $0.02$   & $0.22^{***}$  & $0.23^{***}$  & $0.02$       & $0.02$       \\
                              & $(0.01)$     & $(0.04)$ & $(0.04)$ & $(0.04)$     & $(0.04)$ & $(0.08)$      & $(0.08)$      & $(0.01)$     & $(0.01)$     \\
Log of Pop. Density (t)       & $-0.00^{**}$ & $0.00$   & $0.00$   & $-0.00$      & $0.00$   & $0.01$        & $0.01^{*}$    & $-0.00$      & $-0.00$      \\
                              & $(0.00)$     & $(0.01)$ & $(0.01)$ & $(0.01)$     & $(0.01)$ & $(0.01)$      & $(0.01)$      & $(0.00)$     & $(0.00)$     \\
\hline
Num. obs.                     & $250$        & $300$    & $300$    & $300$        & $300$    & $300$         & $300$         & $250$        & $250$        \\
R$^2$ (full model)            & $0.92$       & $0.18$   & $0.18$   & $0.33$       & $0.19$   & $0.28$        & $0.30$        & $0.93$       & $0.93$       \\
R$^2$ (proj model)            & $0.91$       & $0.01$   & $0.00$   & $0.19$       & $0.01$   & $0.13$        & $0.15$        & $0.91$       & $0.91$       \\
Adj. R$^2$ (full model)       & $0.92$       & $0.16$   & $0.16$   & $0.31$       & $0.16$   & $0.26$        & $0.28$        & $0.92$       & $0.92$       \\
Adj. R$^2$ (proj model)       & $0.91$       & $-0.02$  & $-0.02$  & $0.17$       & $-0.01$  & $0.11$        & $0.12$        & $0.91$       & $0.91$       \\
Num. groups: year             & $5$          & $6$      & $6$      & $6$          & $6$      & $6$           & $6$           & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Within-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:within_epi_2}
\end{center}
\end{table}



==> Supplementary_Tables/Within-EPI-v2.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 \\
\hline
Inequality level (t - 1)          & $-0.21$      &              &              &              &              & $-0.16$      & $-0.24$       & $-0.22$       \\
                                  & $(0.21)$     &              &              &              &              & $(0.21)$     & $(0.21)$      & $(0.21)$      \\
Unemployment (t - 1)              &              & $0.14$       &              &              &              &              & $-0.02$       & $0.06$        \\
                                  &              & $(0.53)$     &              &              &              &              & $(0.52)$      & $(0.49)$      \\
Spatial Within-EP (t - 1)         &              &              & $0.34^{***}$ &              &              &              & $0.31^{**}$   & $0.36^{***}$  \\
                                  &              &              & $(0.12)$     &              &              &              & $(0.14)$      & $(0.14)$      \\
Ed. Attainment (t - 1)            &              &              &              & $-0.15$      &              &              &               & $0.27$        \\
                                  &              &              &              & $(0.17)$     &              &              &               & $(0.20)$      \\
Log of personal Income PC (t - 1) &              &              &              &              & $-0.10^{*}$  & $-0.10^{*}$  & $-0.04$       & $-0.09$       \\
                                  &              &              &              &              & $(0.05)$     & $(0.05)$     & $(0.07)$      & $(0.08)$      \\
Log of GDP PC (t - 1)             & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$  & $0.04^{***}$  \\
                                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$      & $(0.01)$      \\
Log of Pop. Density (t - 1)       & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{***}$ & $-0.02^{***}$ \\
                                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$      & $(0.01)$      \\
\hline
Num. obs.                         & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$         & $250$         \\
R$^2$ (full model)                & $0.38$       & $0.37$       & $0.44$       & $0.38$       & $0.41$       & $0.42$       & $0.45$        & $0.47$        \\
R$^2$ (proj model)                & $0.28$       & $0.28$       & $0.35$       & $0.28$       & $0.32$       & $0.32$       & $0.37$        & $0.38$        \\
Adj. R$^2$ (full model)           & $0.36$       & $0.35$       & $0.42$       & $0.36$       & $0.39$       & $0.40$       & $0.43$        & $0.44$        \\
Adj. R$^2$ (proj model)           & $0.26$       & $0.25$       & $0.33$       & $0.26$       & $0.30$       & $0.30$       & $0.34$        & $0.35$        \\
Num. groups: year                 & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$           & $5$           \\
\hline
\multicolumn{9}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Within-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:within_epi_3}
\end{center}
\end{table}



==> Supplementary_Tables/Within-EPI.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l c c c c c c c c c}
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7 & Model 8 & Model 9 \\
\hline
Within-EP (t - 1)                 & $1.01^{***}$ &              &              &              &              &              &              & $0.99^{***}$ & $0.99^{***}$ \\
                                  & $(0.02)$     &              &              &              &              &              &              & $(0.02)$     & $(0.02)$     \\
Inequality level (t - 1)          &              & $-0.21$      &              &              &              &              & $-0.16$      & $-0.06^{*}$  & $-0.06^{*}$  \\
                                  &              & $(0.21)$     &              &              &              &              & $(0.21)$     & $(0.03)$     & $(0.03)$     \\
Unemployment (t - 1)              &              &              & $0.14$       &              &              &              &              & $-0.21$      & $-0.20$      \\
                                  &              &              & $(0.53)$     &              &              &              &              & $(0.13)$     & $(0.13)$     \\
Spatial Within-EP (t - 1)         &              &              &              & $0.34^{***}$ &              &              &              & $0.04$       & $0.05$       \\
                                  &              &              &              & $(0.12)$     &              &              &              & $(0.03)$     & $(0.03)$     \\
Ed. Attainment (t - 1)            &              &              &              &              & $-0.15$      &              &              &              & $0.02$       \\
                                  &              &              &              &              & $(0.17)$     &              &              &              & $(0.04)$     \\
Log of personal Income PC (t - 1) &              &              &              &              &              & $-0.10^{*}$  & $-0.10^{*}$  & $-0.01$      & $-0.01$      \\
                                  &              &              &              &              &              & $(0.05)$     & $(0.05)$     & $(0.01)$     & $(0.01)$     \\
Log of GDP PC (t - 1)             & $0.00$       & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.04^{***}$ & $0.00^{*}$   & $0.00^{*}$   \\
                                  & $(0.00)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.00)$     & $(0.00)$     \\
Log of Pop. Density (t - 1)       & $-0.00^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.02^{**}$ & $-0.00^{**}$ & $-0.00^{**}$ \\
                                  & $(0.00)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.00)$     & $(0.00)$     \\
\hline
Num. obs.                         & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        & $250$        \\
R$^2$ (full model)                & $0.92$       & $0.38$       & $0.37$       & $0.44$       & $0.38$       & $0.41$       & $0.42$       & $0.93$       & $0.93$       \\
R$^2$ (proj model)                & $0.91$       & $0.28$       & $0.28$       & $0.35$       & $0.28$       & $0.32$       & $0.32$       & $0.91$       & $0.91$       \\
Adj. R$^2$ (full model)           & $0.92$       & $0.36$       & $0.35$       & $0.42$       & $0.36$       & $0.39$       & $0.40$       & $0.92$       & $0.92$       \\
Adj. R$^2$ (proj model)           & $0.91$       & $0.26$       & $0.25$       & $0.33$       & $0.26$       & $0.30$       & $0.30$       & $0.91$       & $0.91$       \\
Num. groups: year                 & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          & $5$          \\
\hline
\multicolumn{10}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level regression analyses of Within-EP as dependent variable. Each regression includes period-fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
\label{tab:within_epi_1}
\end{center}
\end{table}



==> Supplementary_Tables/polarization-manuscript.tex <==

===============================================================================================================================================================
                          Model 1    Model 2    Model 3    Model 4     Model 5    Model 6     Model 7     Model 8     Model 9   Model 10  Model 11   Model 12  
---------------------------------------------------------------------------------------------------------------------------------------------------------------
Inequality level (t)       -0.02                  0.01       0.08       -0.02                   0.02        0.05       -0.00               -0.01       0.06    
                           (0.07)                (0.07)     (0.08)      (0.03)                 (0.03)      (0.04)      (0.06)              (0.07)     (0.07)   
Unemployment (t)                      -0.11 **   -0.12 **   -0.11 **               -0.16 ***   -0.17 ***   -0.09 **               0.03      0.03      -0.05    
                                      (0.04)     (0.04)     (0.05)                 (0.03)      (0.03)      (0.04)                (0.04)    (0.04)     (0.05)   
Polarization (t - 1)                                         0.22 ***                                       0.43 ***                                   0.19 ***
                                                            (0.08)                                         (0.07)                                     (0.05)   
Spatial polarization (t)                                     1.23 ***                                       0.49 ***                                   1.45 ***
                                                            (0.36)                                         (0.12)                                     (0.23)   
Ed. Attainment (t)         -0.05      -0.01      -0.00       0.15        0.27 **    0.33 ***    0.35 ***    0.07       -0.29 *   -0.30 *   -0.30 **    0.11    
                           (0.17)     (0.17)     (0.17)     (0.18)      (0.13)     (0.11)      (0.12)      (0.11)      (0.15)    (0.16)    (0.15)     (0.16)   
Personal Income PC (t)      0.01       0.06       0.05      -0.00        0.25 **    0.33 ***    0.31 ***   -0.02       -0.21 *   -0.23 *   -0.22 *    -0.05    
                           (0.14)     (0.14)     (0.14)     (0.14)      (0.10)     (0.09)      (0.09)      (0.12)      (0.11)    (0.12)    (0.12)     (0.14)   
GDP PC (t)                  0.23 **    0.15       0.15      -0.06        0.08      -0.03       -0.03        0.05        0.15      0.17      0.17      -0.08    
                           (0.09)     (0.09)     (0.10)     (0.11)      (0.08)     (0.08)      (0.08)      (0.07)      (0.11)    (0.11)    (0.11)     (0.12)   
Pop. Density (t)           -0.64      -0.56      -0.59      -1.53        0.04       0.18        0.11       -1.29 **    -0.65     -0.69     -0.66      -0.34    
                           (1.09)     (1.10)     (1.08)     (1.00)      (0.72)     (0.69)      (0.70)      (0.56)      (1.02)    (1.05)    (1.02)     (1.12)   
---------------------------------------------------------------------------------------------------------------------------------------------------------------
Num. obs.                 300        300        300        250         300        300         300         250         300       300       300        250       
R^2 (full model)            0.68       0.68       0.68       0.75        0.88       0.89        0.89        0.94        0.69      0.70      0.70       0.80    
R^2 (proj model)            0.02       0.04       0.04       0.14        0.55       0.59        0.59        0.73        0.25      0.25      0.25       0.44    
Adj. R^2 (full model)       0.60       0.61       0.61       0.67        0.85       0.87        0.87        0.93        0.63      0.63      0.63       0.74    
Adj. R^2 (proj model)      -0.20      -0.18      -0.18      -0.12        0.45       0.50        0.50        0.64        0.08      0.08      0.08       0.27    
Num. groups: state         50         50         50         50          50         50          50          50          50        50        50         50       
===============================================================================================================================================================
*** p < 0.01; ** p < 0.05; * p < 0.1



==> Tables/Associations_Polarization_United_States.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: mer., nov. 30, 2022 - 19:44:41
\begin{table}[H] 
\scriptsize
\centering 
\hspace*{-1cm}


% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: lun., févr. 20, 2023 - 21:03:34

\begin{tabular}{lcccccccccccc}
\hline \hline
Parameters & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\
\hline \hline
Inequality level ($t-1$) & -0.9979*** & -0.0578 &  &  &  &  &  &  & -0.8642*** & -0.0572 & -0.4493*** & -0.0951\\
 & (0.2073) & (0.1219) &  &  &  &  &  &  & (0.1981) & (0.1219) & (0.1514) & (0.1163)\\
Unemployment level ($t-1$) &  &  & -0.1502 & 0.2228 &  &  &  &  &  &  & -0.0904 & 0.1966\\
 &  &  & (0.3875) & (0.2896) &  &  &  &  &  &  & (0.388) & (0.2912)\\
EPI Neighbors level ($t-1$) &  &  &  &  & -0.4665*** & -0.2096*** &  &  &  &  & -0.1198 & -0.1671***\\
 &  &  &  &  & (0.1139) & (0.0618) &  &  &  &  & (0.0848) & (0.0636)\\
EPI level ($t-1$) &  & 0.8334*** &  & 0.6463*** &  & 0.8196*** &  & 0.8257*** &  & 0.8201*** &  & 0.6443***\\
 &  & (0.036) &  & (0.0471) &  & (0.0337) &  & (0.0365) &  & (0.0385) &  & (0.0479)\\
Log of Personal Income ($t-1$) &  &  &  &  &  &  & 0.3666*** & 0.0388 & 0.3315*** & 0.0387 & -0.1002* & -0.0860**\\
 &  &  &  &  &  &  & (0.0647) & (0.0392) & (0.0629) & (0.0393) & (0.0562) & (0.0421)\\
Log of GDP ($t-1$) & -0.2919*** & -0.0608*** & -0.0282 & -0.0100 & -0.3102*** & -0.0662*** & -0.5072*** & -0.0850*** & -0.4730*** & -0.0856*** & 0.0342 & 0.0403\\
 & (0.0226) & (0.016) & (0.024) & (0.0179) & (0.0226) & (0.0157) & (0.0412) & (0.0298) & (0.0405) & (0.0299) & (0.0453) & (0.0339)\\
Population ($t-1$) & 0.3499*** & 0.0685*** & 0.0632** & 0.0197 & 0.3657*** & 0.0758*** & 0.5529*** & 0.0921*** & 0.5243*** & 0.0934*** & 0.0056 & -0.0274\\
 & (0.0225) & (0.0174) & (0.0255) & (0.0192) & (0.0227) & (0.017) & (0.0403) & (0.0305) & (0.0394) & (0.0306) & (0.0454) & (0.0341)\\
\hline \hline
Observations & 245 & 245 & 240 & 240 & 245 & 245 & 245 & 245 & 245 & 245 & 240 & 240\\
Adjusted R2 & 0.576 & 0.87 & 0.218 & 0.567 & 0.566 & 0.876 & 0.591 & 0.87 & 0.62 & 0.87 & 0.248 & 0.579\\
R2 & 0.589 & 0.874 & 0.241 & 0.582 & 0.578 & 0.88 & 0.602 & 0.874 & 0.632 & 0.875 & 0.279 & 0.598\\
Residual Std. Error & 0.087 & 0.048 & 0.061 & 0.045 & 0.088 & 0.047 & 0.085 & 0.048 & 0.082 & 0.048 & 0.06 & 0.045\\
df & 237 & 236 & 232 & 231 & 237 & 236 & 237 & 236 & 236 & 235 & 229 & 228\\
\hline \hline
\end{tabular}


\hspace*{-1cm}
\caption{Socio-demographic characteristics associated to EPI at state level in the United States. Each regression includes period fixed effects. Standard errors in brackets. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.} 
  \label{tab:epi_fixedeffects} 
\end{table} 

==> Tables/Flip_Likelihood.tex <==
\begin{table}[h]
    \scriptsize
    \centering
        \begin{tabular}{llllllll}
        \hline \hline
        Parameters & Model 1 & Model 2 & Model 3 & Model 4 & Model 5 & Model 6 & Model 7\\
        \hline \hline
        Rate Winner & -1.732*** &  &  &  & -2.093*** & -1.884*** & -1.999***\\
         & (0.023) &  &  &  & (0.026) & (0.031) & (0.035)\\
        \hline
        Rate Loser & 1.393*** &  &  &  & 1.631*** & 1.939*** & 1.945***\\
         & (0.021) &  &  &  & (0.023) & (0.031) & (0.033)\\
        \hline
        Divisiveness Winner &  & 0.254*** &  &  & 0.704*** & 0.320*** & 0.349***\\
         &  & (0.01) &  &  & (0.014) & (0.018) & (0.021)\\
        \hline
        Divisiveness Loser &  & -0.248*** &  &  & -0.604*** & -0.064*** & -0.180***\\
         &  & (0.012) &  &  & (0.017) & (0.02) & (0.025)\\
        \hline
        Endorsement Winner &  &  & -0.185*** &  &  & 0.223*** & -0.274***\\
         &  &  & (0.025) &  &  & (0.046) & (0.063)\\
        \hline
        Endorsement Loser &  &  & 1.001*** &  &  & 1.276*** & 1.049***\\
         &  &  & (0.019) &  &  & (0.037) & (0.043)\\
        \hline
        Div. Endors. Winner &  &  &  & -0.375*** &  &  & -0.397***\\
         &  &  &  & (0.024) &  &  & (0.063)\\
        \hline
        Div. Endors. Loser &  &  &  & 0.719*** &  &  & 0.657***\\
         &  &  &  & (0.02) &  &  & (0.038)\\
        \hline
        Same.Winner &  &  &  &  &  &  & 1.247***\\
         &  &  &  &  &  &  & (0.075)\\
        \hline
        Avg. Flip Neighbors &  &  &  &  &  &  & 0.301***\\
         &  &  &  &  &  &  & (0.016)\\
        \hline \hline
        Observations & 68281 & 68281 & 68281 & 68281 & 68281 & 68281 & 68281\\
        \hline
        Deviance & 41573.51 & 51996.75 & 43353.08 & 46410.09 & 37464.43 & 32213.75 & 31314.94\\
        \hline
        Pseudo R2 & 0.22 & 0.02 & 0.18 & 0.13 & 0.29 & 0.39 & 0.41\\
        \hline \hline
        \end{tabular}

    \caption{Comparison of Fixed-Effect Logistic Regressions Models with Country and Year Fixed Effects for \textit{Flipping as Dependant Variable}. Explanatory variables are normalized with SD equal to 0. Values in parenthesis represent standard deviation of coefficients. Note: ***$p<0.01$, **$p<0.05$, *$p<0.1$.}
    \label{tab:flip_likelihood}
\end{table}

==> Tables/between_epi_year.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: dim., févr. 19, 2023 - 23:08:06
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{Between-EPI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Inequality level (t-1) & $-$0.939$^{***}$ &  &  &  & $-$0.733$^{***}$ & $-$0.470$^{***}$ \\ 
  & (0.214) &  &  &  & (0.189) & (0.177) \\ 
  & & & & & & \\ 
 Unemployment level (t-1) &  & 0.429 &  &  &  & 0.871$^{*}$ \\ 
  &  & (0.470) &  &  &  & (0.453) \\ 
  & & & & & & \\ 
 EPI Neighbors (t-1) &  &  & $-$0.258$^{**}$ &  &  & 0.198$^{**}$ \\ 
  &  &  & (0.120) &  &  & (0.099) \\ 
  & & & & & & \\ 
 Log of personal income (t-1) &  &  &  & 0.540$^{***}$ & 0.510$^{***}$ & 0.306$^{***}$ \\ 
  &  &  &  & (0.061) & (0.060) & (0.066) \\ 
  & & & & & & \\ 
 Log of population (t-1) & 0.249$^{***}$ & $-$0.008 & 0.263$^{***}$ & 0.542$^{***}$ & 0.517$^{***}$ & 0.195$^{***}$ \\ 
  & (0.023) & (0.031) & (0.024) & (0.038) & (0.038) & (0.053) \\ 
  & & & & & & \\ 
 Log of GDP (t-1) & $-$0.223$^{***}$ & 0.011 & $-$0.240$^{***}$ & $-$0.530$^{***}$ & $-$0.501$^{***}$ & $-$0.194$^{***}$ \\ 
  & (0.023) & (0.029) & (0.024) & (0.039) & (0.039) & (0.053) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 245 & 240 & 245 & 245 & 245 & 240 \\ 
R$^{2}$ & 0.420 & 0.122 & 0.385 & 0.527 & 0.556 & 0.226 \\ 
Adjusted R$^{2}$ & 0.403 & 0.096 & 0.367 & 0.513 & 0.541 & 0.192 \\ 
Residual Std. Error & 0.090 (df = 237) & 0.074 (df = 232) & 0.092 (df = 237) & 0.081 (df = 237) & 0.079 (df = 236) & 0.070 (df = 229) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> Tables/epi_year.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: dim., févr. 19, 2023 - 23:11:25
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{Within-EPI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Inequality level (t-1) & $-$0.998$^{***}$ &  &  &  & $-$0.864$^{***}$ & $-$0.449$^{***}$ \\ 
  & (0.207) &  &  &  & (0.198) & (0.151) \\ 
  & & & & & & \\ 
 Unemployment level (t-1) &  & $-$0.150 &  &  &  & $-$0.090 \\ 
  &  & (0.388) &  &  &  & (0.388) \\ 
  & & & & & & \\ 
 EPI Neighbors (t-1) &  &  & $-$0.466$^{***}$ &  &  & $-$0.120 \\ 
  &  &  & (0.114) &  &  & (0.085) \\ 
  & & & & & & \\ 
 Log of personal income (t-1) &  &  &  & 0.367$^{***}$ & 0.331$^{***}$ & $-$0.100$^{*}$ \\ 
  &  &  &  & (0.065) & (0.063) & (0.056) \\ 
  & & & & & & \\ 
 Log of population (t-1) & 0.350$^{***}$ & 0.063$^{**}$ & 0.366$^{***}$ & 0.553$^{***}$ & 0.524$^{***}$ & 0.006 \\ 
  & (0.023) & (0.026) & (0.023) & (0.040) & (0.039) & (0.045) \\ 
  & & & & & & \\ 
 Log of GDP (t-1) & $-$0.292$^{***}$ & $-$0.028 & $-$0.310$^{***}$ & $-$0.507$^{***}$ & $-$0.473$^{***}$ & 0.034 \\ 
  & (0.023) & (0.024) & (0.023) & (0.041) & (0.040) & (0.045) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 245 & 240 & 245 & 245 & 245 & 240 \\ 
R$^{2}$ & 0.589 & 0.241 & 0.578 & 0.602 & 0.632 & 0.279 \\ 
Adjusted R$^{2}$ & 0.576 & 0.218 & 0.566 & 0.591 & 0.620 & 0.248 \\ 
Residual Std. Error & 0.087 (df = 237) & 0.061 (df = 232) & 0.088 (df = 237) & 0.085 (df = 237) & 0.082 (df = 236) & 0.060 (df = 229) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> Tables/polarization-manuscript-v2.tex <==

\begin{tabular}{lcccccccccccc}
\hline
Variable & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\
\hline
Inequality level (Gini) (t) & 0.02 & -0.13* & 0.34*** & 0.29*** & -0.20*** & 0.07 & 0.24** & 0.27*** & 0.14*** & -0.20** & 0.24* & 0.19*\\
 & (0.03) & (0.08) & (0.11) & (0.11) & (0.05) & (0.07) & (0.1) & (0.09) & (0.04) & (0.09) & (0.13) & (0.11)\\
Unemployment (t) & 0.05 & -0.17*** & -0.14*** & -0.13** & 0.10* & -0.17*** & -0.06 & -0.02 & -0.01 & -0.09* & -0.12** & -0.10*\\
 & (0.04) & (0.05) & (0.05) & (0.05) & (0.06) & (0.04) & (0.05) & (0.04) & (0.04) & (0.05) & (0.06) & (0.05)\\
Polarization (t - 1) &  &  &  & -0.03 &  &  &  & 0.43*** &  &  &  & 0.05\\
 &  &  &  & (0.07) &  &  &  & (0.08) &  &  &  & (0.07)\\
Spatial polarization (t) &  &  &  & 1.48*** &  &  &  & -0.03 &  &  &  & 2.17***\\
 &  &  &  & (0.4) &  &  &  & (0.15) &  &  &  & (0.3)\\
Ed. Attainment (t) &  &  & 0.03 & 0.18 &  &  & 0.12 & 0.01 &  &  & -0.04 & 0.02\\
 &  &  & (0.25) & (0.24) &  &  & (0.22) & (0.21) &  &  & (0.29) & (0.25)\\
Personal Income PC (t) &  &  & 0.25 & 0.32 &  &  & -0.09 & -0.09 &  &  & 0.35 & 0.21\\
 &  &  & (0.28) & (0.27) &  &  & (0.25) & (0.23) &  &  & (0.33) & (0.29)\\
Expenditure PC (t) &  &  & -0.75** & -0.95*** &  &  & -0.58* & -0.35 &  &  & -0.49 & -0.62\\
 &  &  & (0.37) & (0.36) &  &  & (0.33) & (0.31) &  &  & (0.43) & (0.37)\\
GDP (t) &  &  & -0.43 & -0.53 &  &  & -0.36 & -0.28 &  &  & -0.26 & -0.39\\
 &  &  & (0.33) & (0.32) &  &  & (0.3) & (0.28) &  &  & (0.39) & (0.34)\\
Population (t) &  &  & 1.13 & 1.16 &  &  & 0.94 & 0.58 &  &  & 0.71 & 0.75\\
 &  &  & (0.75) & (0.72) &  &  & (0.67) & (0.62) &  &  & (0.87) & (0.75)\\
Pop. Density (t) &  &  & -5.43 & -8.68* &  &  & -18.10*** & -15.00*** &  &  & 5.18 & -1.17\\
 &  &  & (4.94) & (4.8) &  &  & (4.45) & (4.13) &  &  & (5.78) & (5)\\
\hline
State F.E. &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark\\
Year F.E. &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark\\
\hline
Observations & 300 & 300 & 192 & 192 & 300 & 300 & 192 & 192 & 300 & 300 & 192 & 192\\
Adjusted R2 & 0 & 0.619 & 0.725 & 0.749 & 0.072 & 0.901 & 0.936 & 0.946 & 0.048 & 0.669 & 0.775 & 0.836\\
R2 & 0.006 & 0.69 & 0.809 & 0.828 & 0.078 & 0.919 & 0.955 & 0.963 & 0.054 & 0.731 & 0.843 & 0.888\\
Residual Std. Error & 0.575 & 0.355 & 0.264 & 0.252 & 0.912 & 0.298 & 0.237 & 0.218 & 0.675 & 0.398 & 0.308 & 0.263\\
df & 297 & 243 & 133 & 131 & 297 & 243 & 133 & 131 & 297 & 243 & 133 & 131\\
\hline
\end{tabular}


==> Tables/polarization-manuscript.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lcccccc}
\hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
\hline
Inequality level (t)          & $0.12$      &            &              &             & $0.04$        & $-0.03$      \\
                              & $(0.08)$    &            &              &             & $(0.09)$      & $(0.08)$     \\
Unemployment (t)              &             & $0.16$     &              &             & $0.07$        & $0.12$       \\
                              &             & $(0.10)$   &              &             & $(0.11)$      & $(0.09)$     \\
Within-EP (t)                 &             &            & $0.33^{***}$ &             & $0.40^{***}$  & $0.27^{***}$ \\
                              &             &            & $(0.08)$     &             & $(0.08)$      & $(0.10)$     \\
Between-EP (t)                &             &            &              & $-0.12$     & $0.06$        & $0.02$       \\
                              &             &            &              & $(0.10)$    & $(0.11)$      & $(0.12)$     \\
Inequality * Unemployment (t) &             &            &              &             & $0.03$        & $0.03$       \\
                              &             &            &              &             & $(0.04)$      & $(0.04)$     \\
Spatial Within-EP (t)         &             &            &              &             &               & $0.29^{**}$  \\
                              &             &            &              &             &               & $(0.12)$     \\
Spatial Between-EP (t)        &             &            &              &             &               & $-0.03$      \\
                              &             &            &              &             &               & $(0.11)$     \\
Ed. Attainment (t)            &             &            &              &             & $-0.43^{***}$ & $-0.30^{*}$  \\
                              &             &            &              &             & $(0.16)$      & $(0.15)$     \\
Personal Income PC (t)        &             &            &              &             & $0.19$        & $0.22$       \\
                              &             &            &              &             & $(0.27)$      & $(0.24)$     \\
GDP PC (t)                    &             &            &              &             & $-0.34$       & $-0.22$      \\
                              &             &            &              &             & $(0.34)$      & $(0.27)$     \\
Pop. Density (t)              &             &            &              &             & $0.60^{***}$  & $0.30$       \\
                              &             &            &              &             & $(0.23)$      & $(0.25)$     \\
Swing State                   & $0.34^{**}$ & $0.28^{*}$ & $0.24^{*}$   & $0.39^{**}$ & $0.05$        & $-0.04$      \\
                              & $(0.15)$    & $(0.16)$   & $(0.13)$     & $(0.17)$    & $(0.15)$      & $(0.14)$     \\
\hline
Num. obs.                     & $202$       & $202$      & $202$        & $202$       & $202$         & $202$        \\
R$^2$ (full model)            & $0.37$      & $0.37$     & $0.46$       & $0.37$      & $0.57$        & $0.61$       \\
R$^2$ (proj model)            & $0.04$      & $0.05$     & $0.18$       & $0.04$      & $0.36$        & $0.41$       \\
Adj. R$^2$ (full model)       & $0.35$      & $0.35$     & $0.44$       & $0.35$      & $0.54$        & $0.58$       \\
Adj. R$^2$ (proj model)       & $0.02$      & $0.03$     & $0.16$       & $0.02$      & $0.31$        & $0.36$       \\
Num. groups: year             & $4$         & $4$        & $4$          & $4$         & $4$           & $4$          \\
\hline
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level association of Political Polarization in the United States (2008-2020). Each model represents a multivariate regression, with year-fixed effects. Standard errors are in brackets and are robustly clustered by state. We standardized both independent and dependent variables to have a mean of zero and a standard deviation of one. Note: $***p<0.01$, $**p<0.05$, $*p<0.1$.}
\label{tbl:1}
\end{table}

==> Tables/table_2.tex <==
\begin{table}[H]
\begin{center}
\begin{tabular}{l c c c c c c}
\hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
\hline
Inequality level (t)          & $-0.13$  &             &          &            & $-0.12$      & $-0.15^{*}$  \\
                              & $(0.10)$ &             &          &            & $(0.09)$     & $(0.09)$     \\
Unemployment (t)              &          & $-0.17^{*}$ &          &            & $-0.06$      & $-0.00$      \\
                              &          & $(0.10)$    &          &            & $(0.08)$     & $(0.10)$     \\
Within-EP (t)                 &          &             & $-0.01$  &            & $0.11$       & $0.07$       \\
                              &          &             & $(0.13)$ &            & $(0.16)$     & $(0.11)$     \\
Between-EP (t)                &          &             &          & $0.20^{*}$ & $0.31^{*}$   & $0.23^{**}$  \\
                              &          &             &          & $(0.11)$   & $(0.17)$     & $(0.11)$     \\
Inequality * Unemployment (t) &          &             &          &            & $-0.01$      & $-0.03$      \\
                              &          &             &          &            & $(0.04)$     & $(0.04)$     \\
Spatial Within-EP (t)         &          &             &          &            &              & $-0.04$      \\
                              &          &             &          &            &              & $(0.14)$     \\
Spatial Between-EP (t)        &          &             &          &            &              & $0.22$       \\
                              &          &             &          &            &              & $(0.16)$     \\
Ed. Attainment (t)            &          &             &          &            & $0.53^{***}$ & $0.51^{***}$ \\
                              &          &             &          &            & $(0.15)$     & $(0.15)$     \\
Personal Income PC (t)        &          &             &          &            & $0.08$       & $0.05$       \\
                              &          &             &          &            & $(0.25)$     & $(0.25)$     \\
GDP PC (t)                    &          &             &          &            & $0.11$       & $0.26$       \\
                              &          &             &          &            & $(0.19)$     & $(0.23)$     \\
Pop. Density (t)              &          &             &          &            & $-0.16$      & $-0.33$      \\
                              &          &             &          &            & $(0.25)$     & $(0.21)$     \\
Swing State                   & $0.24$   & $0.30$      & $0.27$   & $0.16$     & $0.30$       & $0.30$       \\
                              & $(0.27)$ & $(0.26)$    & $(0.27)$ & $(0.27)$   & $(0.26)$     & $(0.25)$     \\
\hline
Num. obs.                     & $303$    & $303$       & $303$    & $303$      & $303$        & $303$        \\
R$^2$ (full model)            & $0.27$   & $0.27$      & $0.26$   & $0.30$     & $0.51$       & $0.54$       \\
R$^2$ (proj model)            & $0.03$   & $0.03$      & $0.02$   & $0.07$     & $0.35$       & $0.39$       \\
Adj. R$^2$ (full model)       & $0.26$   & $0.26$      & $0.24$   & $0.28$     & $0.48$       & $0.52$       \\
Adj. R$^2$ (proj model)       & $0.01$   & $0.01$      & $-0.01$  & $0.04$     & $0.31$       & $0.36$       \\
Num. groups: year             & $6$      & $6$         & $6$      & $6$        & $6$          & $6$          \\
\hline
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.01$; $^{**}p<0.05$; $^{*}p<0.1$}}
\end{tabular}
\caption{State-level association of Voting Turnout in the United States (2008-2020). Each model represents a multivariate regression, with year-fixed effects. Standard errors are in brackets and are robustly clustered by state. We standardized both independent and dependent variables to have a mean of zero and a standard deviation of one. Note: $***p<0.01$, $**p<0.05$, $*p<0.1$.}
\label{tbl:2}
\end{center}
\end{table}

==> Tables/within_epi_year.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: dim., févr. 19, 2023 - 23:09:51
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{Within-EPI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Inequality level (t-1) & $-$0.059 &  &  &  & $-$0.131 & 0.021 \\ 
  & (0.139) &  &  &  & (0.136) & (0.126) \\ 
  & & & & & & \\ 
 Unemployment level (t-1) &  & $-$0.579 &  &  &  & $-$0.962$^{***}$ \\ 
  &  & (0.367) &  &  &  & (0.324) \\ 
  & & & & & & \\ 
 EPI Neighbors (t-1) &  &  & $-$0.209$^{***}$ &  &  & $-$0.318$^{***}$ \\ 
  &  &  & (0.074) &  &  & (0.071) \\ 
  & & & & & & \\ 
 Log of personal income (t-1) &  &  &  & $-$0.173$^{***}$ & $-$0.178$^{***}$ & $-$0.406$^{***}$ \\ 
  &  &  &  & (0.043) & (0.043) & (0.047) \\ 
  & & & & & & \\ 
 Log of population (t-1) & 0.101$^{***}$ & 0.071$^{***}$ & 0.103$^{***}$ & 0.011 & 0.007 & $-$0.189$^{***}$ \\ 
  & (0.015) & (0.024) & (0.015) & (0.027) & (0.027) & (0.038) \\ 
  & & & & & & \\ 
 Log of GDP (t-1) & $-$0.069$^{***}$ & $-$0.039$^{*}$ & $-$0.070$^{***}$ & 0.023 & 0.028 & 0.229$^{***}$ \\ 
  & (0.015) & (0.023) & (0.015) & (0.027) & (0.028) & (0.038) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 245 & 240 & 245 & 245 & 245 & 240 \\ 
R$^{2}$ & 0.393 & 0.324 & 0.412 & 0.432 & 0.434 & 0.499 \\ 
Adjusted R$^{2}$ & 0.375 & 0.304 & 0.395 & 0.415 & 0.415 & 0.477 \\ 
Residual Std. Error & 0.058 (df = 237) & 0.057 (df = 232) & 0.057 (df = 237) & 0.056 (df = 237) & 0.056 (df = 236) & 0.050 (df = 229) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
